Process Query Language: Design, Implementation, and Evaluation

Organizations can benefit from the use of practices, techniques, and tools from the area of business process management. Through the focus on processes, they create process models that require management, including support for versioning, refactoring and querying. Querying thus far has primarily focused on structural properties of models rather than on exploiting behavioral properties capturing aspects of model execution. While the latter is more challenging, it is also more effective, especially when models are used for auditing or process automation. The focus of this paper is to overcome the challenges associated with behavioral querying of process models in order to unlock its benefits. The first challenge concerns determining decidability of the building blocks of the query language, which are the possible behavioral relations between process tasks. The second challenge concerns achieving acceptable performance of query evaluation. The evaluation of a query may require expensive checks in all process models, of which there may be thousands. In light of these challenges, this paper proposes a special-purpose programming language, namely Process Query Language (PQL) for behavioral querying of process model collections. The language relies on a set of behavioral predicates between process tasks, whose usefulness has been empirically evaluated with a pool of process model stakeholders. This study resulted in a selection of the predicates to be implemented in PQL, whose decidability has also been formally proven. The computational performance of the language has been extensively evaluated through a set of experiments against two large process model collections.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $< | sed 's/^%\\citestyle{acmauthoryear}/\\citestyle{acmauthoryear}/'      > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> tex/draft_back2sec4-7.tex <==
\newpage

Next, we consider an example process repository consisting of ten process models. 
These models capture business processes that cover various structural features and that are sound. 
They are sourced from the collection of the SAP reference models~\cite{Curran98} as well as from Polyvyanyy's PhD thesis~\cite{Polyvyanyy12}. 
\figurename~\ref{fig:smodels} depicts these ten process models using BPMN. 
Activities are drawn as rectangles with rounded corners. 
Gateways are visualized as diamonds. 
Exclusive gateways use a marker which is shaped like ``$\times$'' inside
the diamond shape, wheres parallel gateways use a marker which is shaped like ``$+$'' inside the diamond shape.
Directed arcs encode control flow dependencies.
For simplicity, the models use only abstract task labels (which are alphabet letters).  

\begin{figure}[hb!]
\centering
\includegraphics[width = 1.0\linewidth]{smodels}
\caption{\small Evaluation of ten sample queries over a repository of ten process models (in BPMN).}
\label{fig:smodels}
\end{figure}

In terms of process structure, the first five models (models~1 to~5) capture acyclic processes and the other five (models~6 to~10) specify processes that contain cycles. Models~1, 2, 6, 7 and~10 are well-structured process models. The others (models~3, 4, 5, 8 and~9) are unstructured process models. Among them, model~4 has a typical Z-structure~\cite{KiepuszewskiHB00}, and models~3 and~5 are two examples of inherently unstructured process models. Model~9 is unstructured but can be mapped to a well-structured model, which is model~10, and both models are equivalent in terms of behavior.  

Next, we propose ten sample queries over the set of PQL constructs. 
These capture the six atomic behavioral predicates (which are selected according to our empirical evaluation in \sectionname~\ref{subsec:empirical:evaluation:results}), %supported by the first edition of PQL), 
the corresponding predicate macros, logical operations over predicates and predicate macros, construction of task sets using predicates, set operations, and set comparison operations, \see\sectionname~\ref{subsec:PQL:abstract:syntax}). 
These sample queries (named \textit{Q1}--\textit{Q10}), as listed below, are instantiations of ten query templates out of a total of 150 query templates to be used for evaluation of PQL in Section~\ref{sec:dataset}. 

\newpage

Querying scenarios and PQL query statements over the process repository in Figure~\ref{fig:smodels}.

from the process model repository ``Ten-Models-BPMN'' in the folder called ``ProcessRepo''

\medskip
\begin{itemize}
	% 1 ------------------------------------- %
	\item[\textit{S1}.] \emph{Retrieve the IDs of all process models where D occurs in at least one process instance} 
							\item[] \emph{and it never occurs in the same instance as E} \\ 
	\vspace*{-.75\baselineskip}
	\item[\textit{Q1}.] \texttt{\SELECT~"ID" \FROM~"/ProcessRepo/Ten-Models-BPMN"} 
							\item[] \texttt{\WHERE~CanOccur("D")~\AND~Conflict("D","E");} \\
	\vspace*{-.5\baselineskip}
	% 2 ------------------------------------- %
	\item[\textit{S2}.] \emph{Retrieve the IDs of all process models where C occurs in every process instance} 
							\item[] \emph{or it always occurs in the same instance as B and vice versa} \\ 
	\vspace*{-.75\baselineskip}
	\item[\textit{Q2}.] \texttt{\SELECT~"ID" \FROM~"/ProcessRepo/Ten-Models-BPMN"} 
							\item[] \texttt{\WHERE~AlwaysOccurs("C")~\OR~Cooccur("B","C");} \\
	\vspace*{-.5\baselineskip}
	% 3 ------------------------------------- %
	\item[\textit{S3}.] \emph{Retrieve the IDs and titles of all process models where} 
							\item[] \emph{1) G occurs in at least one process instance and it may occur in the same instance as E, or} 
							\item[] \emph{2) D occurs in every process instance and it always occurs concurrently with C} \\ 
	\vspace*{-.75\baselineskip}
	\item[\textit{Q3}.] \texttt{\SELECT~"ID","Title" \FROM~"/ProcessRepo/Ten-Models-BPMN"} 
							\item[] \texttt{\WHERE~(CanOccur("G")~\AND~(\NOT~Conflict("E","G")))~\OR~} 
							\item[] \texttt{\hspace{10.3mm}(AlwaysOccurs("D")~\AND~TotalConcurrent("C","D"));} \\
	\vspace*{-.5\baselineskip}
	% 4 ------------------------------------- %
	\item[\textit{S4}.] \emph{Retrieve the IDs and titles of all process models where, for F and G, each of them occurs} 
							\item[] \emph{in at least one process instance, and at least one of them occurs in every process instance} \\ 
	\vspace*{-.75\baselineskip}
	\item[\textit{Q4}.] \texttt{\SELECT~"ID","Title" \FROM~"/ProcessRepo/Ten-Models-BPMN"} 
							\item[] \texttt{\WHERE~CanOccur(\{"F","G"\},\ALL)~\AND~AlwaysOccurs(\{"F","G"\},\ANY);}\\ 
	\vspace*{-.5\baselineskip}
	% 5 ------------------------------------- %
	\item[\textit{S3}.] \emph{Retrieve the IDs and titles of all process models where} 
							\item[] \emph{1) G occurs in at least one process instance and it may occur in the same instance as E, or} 
							\item[] \emph{2) D occurs in every process instance and it always occurs concurrently with C} \\ 
	\vspace*{-.75\baselineskip}
	\item[\textit{Q3}.] \texttt{\SELECT~"ID","Title" \FROM~"/ProcessRepo/Ten-Models-BPMN"} 
							\item[] \texttt{\WHERE~CanOccur(\{"F","G"\},\ALL)~\AND~AlwaysOccurs(\{"F","G"\},\ANY);}\\ 
	\vspace*{-.5\baselineskip}
	\vspace*{-.75\baselineskip}
	\item[\textit{Q5}.]\ \texttt{\SELECT~* \FROM~*} 
	\item[]\hspace{3.3mm}\texttt{\WHERE~Cooccur("B",\{"C","D"\},\ALL)~\AND~TotalConcurrent("B",\{"C","D"\},\ANY);}\\
\end{itemize}
\medskip


\medskip
%\footnotesize
\begin{itemize}
	\item[\textit{Q1}.]\ \texttt{\SELECT~* \FROM~* \WHERE~CanOccur("D")~\AND~Conflict("D","E");}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q2}.]\ \texttt{\SELECT~* \FROM~* \WHERE~AlwaysOccurs("C")~\OR~Cooccur("B","C");}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q3}.]\ \texttt{\SELECT~* \FROM~*} 
	\item[]\hspace{3.3mm}\texttt{\WHERE~(CanOccur("G")~\AND~(\NOT~Conflict("E","G")))~\OR~}
	\item[]\hspace{3.3mm}\texttt{(TotalConcurrent("C","D")~\AND~AlwaysOccurs("D"));}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q4}.]\ \texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~CanOccur(\{"F","G"\},\ALL)~\AND~AlwaysOccurs(\{"F","G"\},\ANY);}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q5}.]\ \texttt{\SELECT~* \FROM~*} 
	\item[]\hspace{3.3mm}\texttt{\WHERE~Cooccur("B",\{"C","D"\},\ALL)~\AND~TotalConcurrent("B",\{"C","D"\},\ANY);}\\
	\vspace*{-.75\baselineskip} 
	\item[\textit{Q6}.]\ \texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~Conflict(\{"A","B"\},\{"E","F"\},\ANY)~\OR~}
	\item[]\hspace{3.3mm}\texttt{(Cooccur(\{"A","B"\},\{"E","F"\},\EACH)~\AND~}
	\item[]\hspace{3.3mm}\texttt{TotalCausal(\{"A","B"\},\{"E","F"\},\ALL));}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q7}.]\ \texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~"C"~\IN~(GetTasksAlwaysOccurs(\{"C"\})~\UNION~}	
	\item[]\hspace{3.3mm}\texttt{GetTasksTotalCausal(\{"C"\},\{"B","D"\},\ALL));}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q8}.]\ \texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~"G"~\IN~(GetTasksCanOccur(\{"G"\})~\INTERSECT~}	
	\item[]\hspace{3.3mm}\texttt{GetTasksConflict(\{"G"\},\{"D","E","F"\},\ANY));}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q9}.]\ \texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~GetTasksCooccur(\{"A","B","C"\},\{"D","E"\},\ANY)~\NOT~\EQUALS~}	
	\item[]\hspace{3.3mm}\texttt{GetTasksTotalConcurrent(\{"A","B","C"\},\{"D","E"\},\ANY);}\\
	\vspace*{-.75\baselineskip}
	\item[\textit{Q10}.]\hspace{-.9mm}\texttt{\SELECT~* \FROM~*}
	\item[]\hspace{3.3mm}\texttt{\WHERE~(\{"A","B","E","F"\}~\EXCEPT~}
	\item[]\hspace{3.3mm}\texttt{GetTasksCooccur(\{"A","B","E","F"\},\{"C","D"\},\ALL))~\OVERLAPS~\WITH~}
	\item[]\hspace{3.3mm}\texttt{GetTasksConflict(\{"A","B","E","F"\},\{"C","D"\},\ANY);}
\end{itemize}
\medskip

%In order to illustrate the formal semantics of APQL, a number of process models, represented in BPMN, are presented in Fig. 4. For each sample query of Section 2.3 and for each model it is indicated whether the model is part of the answer to the query (in that case the box corresponding to the query is ticked otherwise the box is not ticked). Note that in some models tasks with the same label occur (e.g. there are two tasks labeled A in model f), in which case, APQL will treat these tasks as same tasks during query evaluation.\footnote{}

We apply the above ten sample queries to the collection of ten process models shown in \figurename~\ref{fig:smodels}. Each query is evaluated over these ten individual process models according to the semantics of PQL (defined in Sections~\ref{subsec:PQL:dynamic:semantics} and~\ref{subsec:PQL:predicates:semantics}). The evaluation result indicates whether a process model satisfies the condition specified in the \WHERE~clause of a specific query. In \figurename~\ref{fig:smodels}, this is depicted by a query name being ticked or not ticked under each process model. For each query, only the process models that satisfy the \WHERE~condition of the query are retrieved as the answer to the query. Table~\ref{tab:squeryrslt} summarizes the answers to the ten individual sample queries over the collection of these ten process models. Since models~9 and~10 are behaviorally equivalent, any query evaluation over these two models yields the same result. 

\begin{table}[b]
\footnotesize
  \centering
  \caption{\small Answers to ten sample queries over the collection of ten process models in \figurename~\ref{fig:smodels}.} 
		\begin{tabular}{| l | l || l | l |}
		\hline
		\textbf{Query Id.} & \textbf{Answer to query (set of models)} & \textbf{Query Id.} & \textbf{Answer to query (set of models)} \\
		\hline 
		\hline 
		\textit{Q1} & \{1, 5\} & 
		\textit{Q6} & \{1, 2, 3\} \\
		\hline 
		\textit{Q2} & \{1, 4, 6, 7, 9, 10\} & 
		\textit{Q7} & \{1, 2, 3, 4, 7, 9, 10\} \\
		\hline 
		\textit{Q3} & \{4, 6, 7, 9, 10\} & 
		\textit{Q8} & \{8\} \\
		\hline 
		\textit{Q4} & \{6, 9, 10\} & 
		\textit{Q9} & \{3, 4, 5, 6, 7, 9, 10\} \\
		\hline 
		\textit{Q5} & \{4, 9, 10\} & 
		\textit{Q10} & \{1, 2, 3, 5, 6\} \\
		\hline 
\end{tabular}
\label{tab:squeryrslt}
\end{table}

%--- Add some insights ---

Now let's consider a couple of examples among the ten sample queries. Query~\textit{Q1} is designed to retrieve those process models where 1) task labeled~\texttt{"D"} (task~\texttt{D} for short) occurs in at least one process instance (\texttt{CanOccur("D")}) and 2) there is no process instance in which tasks~\texttt{D} and~\texttt{E} both occur (\texttt{Conflict("D","E")}). The first condition holds in all models in \figurename~\ref{fig:smodels}, while the second condition holds in models~1 and~5 only. It is important to understand the behavior of a process model when evaluating the second condition. For example, in model~8, although tasks~\texttt{D} and~\texttt{E} are on two exclusive branches (subsequent to task~\texttt{B}), both tasks may occur in one process instance since task~\texttt{D} is part of a cycle that loops back to task~\texttt{B}. Another interesting example concerns query~\textit{Q3}, in particular, the condition \texttt{TotalConcurrent("C","D")} in the query. This condition holds for a process model, if and only if for every instance in which tasks~\texttt{C} and~\texttt{D} both occur, every occurrence of task~\texttt{C} can be executed at the same time with every occurrence of task~\texttt{D}. For certain process models, such as model~3, due to the characteristics of this unstructured model, it would not be possible to evaluate this condition without knowledge of the model's behavior.%al information.

%satisfy the second condition thus becoming the results of Q1. ... the second condition, and hence Q1 retrieves  . It is interesting to examine model~8 for evaluation of condition~2,   
%More precisely, it would not be possible to express that $e_8$ is concurrent with all occurrences of $f_7$ as the latter is part of a cycle. 
%For example, given the collection of process models in \figurename~\ref{fig:smodels}, the answer to query~Q1 is the set of models~1 and~5, and the answer to query~Q10 is the set of models~1, 2, 3, 5 and~6.   

%(To be completed ...) 
%It will be wise to focus on some examples of evaluating a certain query over a certain model that requires the understanding of the behavioural semantics of the model. Possible examples: Conflict(D,E) on model 8, TotalConcurrent(C, D) or TotalConcurrent(B,{C,D},xxx) on model 3, etc.
% 
%[Old draft] Let's consider two examples. One is about query~Q2. It is designed to find those process models where in every instance of such a process 1) task~\texttt{"C"} occurs (by predicate \texttt{AlwaysOccur("C")}), or, 2) the two tasks~\texttt{"B"} and~\texttt{"C"} either both occur or neither occurs (by predicate \texttt{Cooccur("B","C")}). In Fig.~\ref{fig:smodels}, models~1, 4, 7, 9,~10 satisfy the first condition as in the rest of the models task~\texttt{"C"} is on a conditional branch. 

%\small
%\begin{equation}
%\texttt{\SELECT~* \FROM~* \WHERE~CanOccur("D")~\AND~Conflict("D", "E");}
%\end{equation}
%\normalsize
%\vspace*{-\baselineskip}
%
%\small
%\begin{equation}
%\texttt{\SELECT~* \FROM~* \WHERE~AlwaysOccur("C")~\OR~Cooccur("B", "C");}
%\end{equation}
%\normalsize
%
%\small
%\begin{equation}
%\begin{split}
%&\texttt{\SELECT~* \FROM~*}\\
%&\texttt{\WHERE~CanCooccur("Check credit","Check character"[0.95]);}
%\end{split}
%\end{equation}
%\normalsize
%
%\small
%\begin{equation}
%\begin{split}
%&\texttt{\SELECT~* \FROM~"BIT"}\\
%&\texttt{\WHERE~AlwaysOccurs(\{"Check credit"[.9],"Check character"\},\ALL);}
%\end{split}
%\end{equation}
%\normalsize
%
%\small
%\begin{equation}
%\texttt{\SELECT~id \FROM~"BIT" \WHERE~\NOT~CanOccur(*,\ALL);}
%\end{equation}
%\normalsize
%
%\small
%\begin{equation}
%\begin{split}
%& \texttt{x\! =\! \{"A","B"\};}\\
%& \texttt{y\! =\! \{"X","Y","Z"\};}\\
%& \SELECT~\texttt{*}~\FROM\;\;\texttt{1001\!,\,1002\!,\,1003}\\
%& \WHERE~\texttt{GetTasksAlwaysOccurs(*)}~\IS~\SUBSET~\OF~\texttt{x}~\AND\\
%& \texttt{ExistentialConcurrent(x,y,\ANY);}
%\end{split}
%\end{equation}
%\normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex/empirical_study.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Empirical Study}
\label{sec:empirical}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

which sort of questions you typically have to answer about processes that exist in your organization

The data collection will be conducted through interviews and/or focus groups. The participants are drawn from professionals who deal with business process models, and in general with BPM initiatives, in their daily activities. The purpose of this research is to understand what type of information you would need to know from your process models, and thus to formulate a query language you can use to query your process model repository.
Your participation in this project is entirely voluntary. If you do not agree to participate, you can withdraw from the project without comment or penalty. If you withdraw, on request any identifiable information already obtained from you will be destroyed. Your decision to participate, or not participate, will in no way impact upon your current or future relationship with QUT or your organization.
Your participation will involve an interview or the participation in a focus group at your organization, and will take approximately 60 min of your time. We have derived a set of core question types that can be asked when querying process model repositories. While guided by these core questions, this instrument will also allow you to express your own views and concerns on the topic.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interviews}
\label{sec:interviews}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The interview is given in Appendix~\ref{app:PQL:interview}.

We have conducted 10 interviews.

Total length of recorded audio materials 619 min and 55 sec.

Discuss demographics, i.e, roles people were involved and for how many years, etc. 

Motivate selection of primitives via 4C spectrum. We want to cover different types of relations for different strengths. Interview should be not long, preferably approx. 1h.

We were discussing primitives in detail, asking participants to answer several questions to guarantee understanding of the primitives.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Selecting Query Primitives}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Wikipedia: All programming languages have some \emph{primitive} building blocks for the description of data and the processes or transformations applied to them (like the addition of two numbers or the selection of an item from a collection). These primitives are defined by syntactic and semantic rules which describe their structure and meaning respectively.


Double result: first, we show that indeed behavioral predicates are perceived as being useful, important, and that they are likely to occur in practice and are frequently observed. Second, we selected those to implement: here Total ranks the highest


\begin{figure}
\begin{center}
  \subfigure[]{\label{fig:plot:useful:important}\includegraphics[width = .48\linewidth]{plot/useful-important}}
  \subfigure[]{\label{fig:plot:useful:likely}\includegraphics[width = .48\linewidth]{plot/useful-likely}}
	\subfigure[]{\label{fig:plot:useful:frequent}\includegraphics[width = .48\linewidth]{plot/useful-frequent}}
	\subfigure[]{\label{fig:plot:important:likely}\includegraphics[width = .48\linewidth]{plot/important-likely}}
	\subfigure[]{\label{fig:plot:important:frequent}\includegraphics[width = .48\linewidth]{plot/important-frequent}}
	\subfigure[]{\label{fig:plot:likely:frequent}\includegraphics[width = .48\linewidth]{plot/likely-frequent}}
\end{center}
\vspace{-3mm}
\caption{TODO.}
\label{fig:behavioral:relations}
\vspace{-3mm}
\end{figure}

Summary from the cross-tab analysis after selecting 6 best sums of respective dimensions:
\texttt{CanOccur} (6), \texttt{AlwaysOccurs} (6), \texttt{Cooccur} (6), \texttt{Conflict} (5), \texttt{ExistTotalCausal} (2), \texttt{TotalExistCausal} (1), \texttt{TotalCausal} (6), \texttt{TotalExistConcurrent} (2), \texttt{TotalConcurrent} (6).
Note that there are more than $6 \times 6$ scores as for some crosstabs there were several behavioral primitives that scored the same value.
Also note that \texttt{ExistTotalCausal}, \texttt{TotalExistCausal}, \texttt{TotalExistConcurrent} labels are not shown in the cross-tab plots; though they are shown with black dots.

\setlength\extrarowheight{2pt}

\begin{table}[htbp]
\footnotesize
  \centering
  \caption{TODO}
\begin{tabular}{r|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-13}
& \rotatebox[origin=l]{90}{\texttt{\textbf{CanOccur}}\;\;} & \rotatebox[origin=l]{90}{\texttt{\textbf{AlwaysOccurs}}\;\;} & \rotatebox[origin=l]{90}{\texttt{\textbf{Cooccur}}\;\;} & \rotatebox[origin=l]{90}{\texttt{\textbf{Conflict}}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistTotalCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalExistCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{\textbf{TotalCausal}}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistTotalConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalExistConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{\textbf{TotalConcurrent}}\;\;} \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Useful} } & 4.0   & 3.6   & 3.7   & 3.7   & 3.3   & 3.4   & 3.6   & 3.9   & 3.0   & 3.2   & 3.6   & 3.9 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Important} } & 3.8   & 3.4   & 3.4   & 3.6   & 3.3   & 3.3   & 3.4   & 3.8   & 3.1   & 3.0   & 3.3   & 3.5 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Likely} } & 4.4   & 3.4   & 3.8   & 3.5   & 2.9   & 3.4   & 3.4   & 3.3   & 3.4   & 3.2   & 3.1   & 3.4 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Frequent} } & 3.5   & 3.2   & 3.2   & 2.9   & 2.6   & 2.9   & 2.9   & 3.1   & 2.6   & 2.8   & 3.0   & 3.2 \\
\hline
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Sum} }   & \textbf{15.7} & \textbf{13.6} & \textbf{14.1} & \textbf{13.7} & 12.1  & 13.0  & 13.3  & \textbf{14.1} & 12.1  & 12.2  & 13.0    & \textbf{14.0}\\
\hline
    \end{tabular}
  \label{tab:interview:averages}
\end{table}

\begin{table}[htbp]
\footnotesize
  \centering
  \caption{TODO}
\begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{3cm}|}
\hline
How \textbf{useful} would an answer to such a question type be for your process analysis work? & How \textbf{important} is such a question type to your process analysis work? & During process analysis, how \textbf{likely} does such a question type occur? & During process analysis, how \textbf{frequently} does such a question type occur? \\
\hline
1 -- Not at all useful\newline
2 -- Slightly useful\newline
3 -- Moderately useful\newline
4 -- Very useful\newline
5 -- Extremely useful
& 
1 -- Not at all important\newline
2 -- Slightly important\newline
3 -- Moderately important\newline
4 -- Very important\newline
5 -- Extremely important
&
1 -- Extremely unlikely\newline
2 -- Unlikely\newline
3 -- Neutral\newline
4 -- Likely\newline
5 -- Extremely likely
&
1 -- Never\newline
2 -- Almost never\newline
3 -- Occasionally\newline
4 -- Almost every time\newline
5 -- Always
\\
\hline
    \end{tabular}
  \label{tab:interview:scale}
\end{table}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tex/old-stuff.tex <==
\subsection{Process Definition}

Using an illustrative example (a simple order-to-cash process adopted from FBPM book) to introduce the concepts of:
\begin{itemize}
	\item business process
	\item three perspectives of a business
	\item process model (\& modelling languages)
	\item ?
\end{itemize}

A business process is a collection of inter-related events, activities and decision points that involve a number of actors and objects, and that collectively lead to an outcome that is of value to at least one customer. 

\begin{figure}[h]
	\centering
		\vspace{-.75em}
		\includegraphics[width=0.7\textwidth]{order-to-cash-bpmn.pdf}
	\caption{A simple order to cash process (modelled in BPMN)}
	\vspace{-1.5em}
	\label{fig:order-to-cash-bpmn}
\end{figure}

Control-flow: A typical order-to-cash process is triggered by the receipt of a purchase order (from a customer). 
The purchase order has to be checked against the stock regarding the availability of the item(s) requested. 
Depending on stock availability the purchase order may be confirmed or rejected. 
If the purchase order is confirmed, an invoice is emitted and the goods requested are shipped. 
The process completes by archiving the order or if the order is rejected.

Data perspective: The purchase order document serves as an input to the stock availability check. 
Based on the outcome of this check, the status of the document is updated, either to ``approved'' or ``rejected''. 
If the order is approved, an invoice and a shipment notice are produced.

Resource perspective: The above process is carried out by a seller's organization which includes two departments: the Sales department and the Warehouse \& Distribution department. 
The purchase order received by the Sales department has to be checked against the stock. 
This is done via an ERP module within the Warehouse \& Distribution department. 
If the purchase order is confirmed, the Warehouse \& Distribution department ships the goods. Meantime, the Sales department emits the invoice. The process concludes with the order being archived by the Sales department. 


\subsection{Process Execution}

%Is there an existing meta-model of process execution (hence for consistency with terminologies)? 

To introduce run-time concepts of a business process: 
\begin{itemize}
	\item process instance (\ie case)
	\item activity instance (\ie work item) 
	\item action/operation (\& modelling languages)
	\item ?
\end{itemize}

\footnote{The term business process management system (BPMS) is often used to refer to something similar to a workflow management system. The difference is that a BPMS supposedly offers richer functionality for analysing business processes, while workflow systems traditionally focused on the co-ordination of tasks. However, the gap between these two is narrowing, and it is difficult to differentiate modern workflow management systems and BPMSs~\cite{}.}

Work item lifecycle (taking into account resource interactions) 
TO DO: Incl. a transition arc from Created to Started (for automated task)

Figure of work item lifecycle

\subsection{Business Process Management System}

WfMS Reference Model

What is a generic/standard structure of a business process automation system (previously known as )

\begin{itemize}
	\item Three perspectives of a process: control flow, data and resource 
	\item Resource handling is one of the key functionalities of a modern business process automation system
	\item Complex resource interactions as conceptually captured by a set of Resource Pat-terns
	\item The BPM reference architecture (reference model of WfMC) considers resource handling as the responsibilities of workflow engines. 
	\item No specific consideration has been given to resource handling in that reference model, despite the evolved complexity of resource interactions and the necessary support 
	\item The BPA / WfMS that we are interested in has many human interactions, i.e. inter-actions with human resources, etc.  
	\item Existing BPM systems, except YAWL, often give little or inadequate support to re-source handling. (from the evaluation of BPM tools?)
\end{itemize}

==> tex/predicates3.tex <==
% !TEX root = ../tods.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Query Predicates and their Relevance}
\label{sec:behavioral:relations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section introduces a set of predicates to specify different behavioral inter-task dependencies in a process models query language. Next, the section sheds light on the practical relevance of these behavioral predicates by reporting on the results of an empirical experiment with process models experts. The results are then used to inform the selection of the predicates to implement in our query language.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Behavioral Predicates}
\label{sec:predicates}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Marcello, let me know if you want to change something in the first paragraph

A \emph{behavioral predicate} is a finitary relation over process tasks that specifies ordering constraints for possible occurrences of the tasks.
It is known that binary relations of \emph{conflict}, \emph{causality}, and \emph{concurrency} can be used to describe any ``behavior'' model, where a behavior model is a process model that explicitly represents repeating states, refer to~\cite{SassoneNW96} for details.
An occurrence of a process task of a behavior model implies that all its causally dependent tasks have already occurred and none of the conflicting tasks has been or will be observed, whereas two concurrent tasks of a behavior model can be enabled for a simultaneous execution.
Recently, the reveals relation has been introduced to capture the phenomenon of \emph{co-occurrence} of process tasks in behavior models~\cite{HaarKS13}, where, intuitively, two process tasks co-occur if they both occur in an instantiation of the process model. 
However, it is also well-known that a behavior model which specifies that a certain process state can be reached infinitely often is infinite!
Therefore, in practice, process analysts mostly work with ``system'' models, where a system model, as per the classification in~\cite{SassoneNW96}, is a finite process model that implicitly encodes states that can be reached infinitely many times. 
EPCs and Petri net systems are examples of system models.
For example, the system in \figurename~\ref{fig:system} prescribes that the marking that puts one token at place $p_5$, one token at place $p_{11}$, one token at place $c_4$, and no tokens elsewhere, can be reached infinitely often.

% Marcello, text below can be improved

The \emph{4C spectrum}~\cite{PolyvyanyyWCRH14} is a systematic classification of behavioral predicates that target description of system models and are grounded in the four fundamental behavioral phenomena mentioned above.
It proposes 18 basic relations over process tasks that can be combined using logical connectives into 318 behavioral predicates that explore conflict (63 predicates), co-occurrence (15), causality (120), and concurrency (120) phenomena at different levels of granularity (given two process tasks, assess whether in all/some instances of the model all/some occurrence of one task are in relation with all/some occurrences of the other task).

To assess the relevance of using behavioral predicates for the purpose of querying process model collections, we decided to use a subset of the predicates of the 4C spectrum. 
The selection of the predicates was driven by three factors: 
(i) the selected predicates must cover all the four behavioral phenomena, 
(ii) the selected predicates must cover predicates of different granularity, and 
(iii) the list of the selected predicates must be concise.
At the end, we have selected ten 4C predicates: one conflict, one co-occurrence, four causality, and four concurrency predicates.
The reason behind selecting only one conflict predicate and only one co-occurrence predicate is that all the 63 conflict and 15 co-occurrence predicates of the 4C spectrum stem form logical expressions over two basic relations that address the respective behavioral phenomena.
Four causal and four concurrent predicates were selected from eight basic causal relations and eight basic concurrency relations, respectively.
The selected predicates explore the different granularity of causality and concurrency offered by the 4C spectrum, \eg given two process tasks, assess whether in all instances of the model all occurrence of one task are concurrent causal with all occurrences of the other task.
%Note that the selected ten predicates can be used to express half of the 4C spectrum predicates.
In addition, we included two unary behavioral predicates that can be used to check whether a given process task can occur or always occurs in instances of a process model~\cite{HofstedeORS0P13,PolyvyanyyRH14}.

% Marcello, I do not know what can we say here. I do not know why, but we no longer have a reference to the APQL paper. Maybe this was our angle here. We reused the two APQL unary relations form our previous works?

\tablename~\ref{tab:predicates} lists the twelve selected predicates. 
Note that the textual descriptions of the predicates are already adjusted to specify intents to retrieve relevant process models from a collection thereof.

\begin{table}[htbp]
\footnotesize
  \centering
\begin{tabular}{|r|p{9.2cm}|}
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{\textbf{Behavioral predicate}} }  & \multicolumn{1}{ |l|  }{\multirow{1}{*}{\textbf{Definition}} } \\
\hline
\hline
\texttt{CanOccur(A)}\!\! & Find all process models where task \textbf{A} occurs in \emph{at least one} instance. \\
\hline
\texttt{AlwaysOccurs(A)}\!\! & Find all process models where task \textbf{A} occurs in \emph{every} instance. \\
\hline
\texttt{Cooccur(A,B)}\!\! & Find all process models where it holds that if task \textbf{A} occurs in \emph{some} instance then task \textbf{B} occurs in the \emph{same} instance, and \emph{vice versa}. \\
\hline
\texttt{Conflict(A,B)}\!\! & Find all process models where it holds that there is \emph{no} instance in which tasks \textbf{A} and \textbf{B} \emph{both} occur. \\
\hline
\texttt{ExistCausal(A,B)}\!\! & Find all process models where in \emph{at least one} instance it holds that \emph{some} occurrence of task \textbf{A} precedes \emph{some} occurrence of task \textbf{B}. \\
\hline
\texttt{ExistTotalCausal(A,B)}\!\! & Find all process models where in \emph{at least one} instance it holds that tasks \textbf{A} and \textbf{B} both occur, and \emph{every} occurrence of task \textbf{A} precedes \emph{every} occurrence of task \textbf{B}. \\
\hline
\texttt{TotalExistCausal(A,B)}\!\! & Find all process models where for \emph{every} instance in which tasks \textbf{A} and \textbf{B} \emph{both} occur, it holds that \emph{some} occurrence of task \textbf{A} precedes \emph{some} occurrence of task \textbf{B}. \\
\hline
\texttt{TotalCausal(A,B)}\!\! & Find all process models where for \emph{every} instance in which tasks \textbf{A} and \textbf{B} \emph{both} occur, it holds that \emph{every} occurrence of task \textbf{A} precedes \emph{every} occurrence of task \textbf{B}. \\
\hline
\texttt{ExistConcurrent(A,B)}\!\! & Find all process models where in \emph{at least one} instance it holds that \emph{some} occurrence of task \textbf{A} can be executed at the same time with \emph{some} occurrence of task \textbf{B}. \\
\hline
\texttt{ExistTotalConcurrent(A,B)}\!\! & Find all process models where in \emph{at least one} instance it holds that tasks \textbf{A} and \textbf{B} \emph{both} occur, and \emph{every} occurrence of task \textbf{A} can be executed at the same time with \emph{every} occurrence of task \textbf{B}. \\
\hline
\texttt{TotalExistConcurrent(A,B)}\!\! & Find all process models where for \emph{every} instance in which tasks \textbf{A} and \textbf{B} both occur, it holds that \emph{some} occurrence of task \textbf{A} can be executed at the same time with \emph{some} occurrence of task \textbf{B}. \\
\hline
\texttt{TotalConcurrent(A,B)}\!\! & Find all process models where for \emph{every} instance in which tasks \textbf{A} and \textbf{B} \emph{both} occur, it holds that \emph{every} occurrence of task \textbf{A} can be executed at the same time with  \emph{every} occurrence of task \textbf{B}. \\
\hline
    \end{tabular}
  \label{tab:behavioral:primitives}\caption{The twelve behavioral predicates chosen for the empirical assessment.}\label{tab:predicates}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiment Design}
\label{subsec:empirical:evaluation}

% Using these twelve predicates, we designed an experiment aimed at answering the following two questions:
% \begin{enumerate}
% \item Does the use of such predicates in a behavioral query language target a practical problem?
% \item Which predicates would be particularly relevant in practice?
% \end{enumerate}
%
% While the first question helps us clarify the practical relevance of behavioral querying of process model collections, the second question was used to drive the selection of which predicates to implement in our language.

We prepared an experiment with two aims: i) help us gain an understanding of the practical relevance of behavioral querying of process model collections, using the twelve predicates identified above, and ii) drive the selection of which predicates to implement in our query language. The experiment took the form of a one-hour interview to seek expert opinion from practitioners that actively work with process model collections. The practitioners were contacted through public posting in dedicated LinkedIn groups (e.g.\ in the areas of business process management and process mining), or approached directly using our industry network. 

As part of the interview, we first explained the rationale of the experiment and introduced the notion and main characteristics of a process model query language. Next, we showed each of the twelve predicates in Table~\ref{tab:predicates} through a simple example, and conducted a short test to ensure that the interviewee had grasped the meaning of each predicate. Each predicate was presented in the form of a ``type of question'' that a process stakeholder such as a business analyst may need to get an answer for, about the process models that exist in their organization. For example, for the unary predicate CanOccur, we used the question ``Find all process models where task \textbf{A} occurs in \emph{at least one} instance'', while for the binary predicate Conflict we used ``Find all process models where it holds that there is \emph{no} instance in which tasks \textbf{A} and \textbf{B} both occur''.

We then proceeded with the actual questionnaire, which was divided into three parts. In the first part, we collected demographic information on the participants, such as role and experience with process models management. The latter revolved around the number and type of process models managed, the key problems faced with these models, and the extent of process analysis conducted on these models on a daily basis. 

Next, we used four established metrics of data quality (usefulness, importance, likelihood and frequency) as proxies for relevance, by asking the following four questions for each predicate, using a 5-point Likert scale for the answer:

\begin{itemize}
	\item How \textbf{useful} would an answer to such a question type be for your process analysis work?
	\item How \textbf{important} is such a question type to your process analysis work? 
	\item During process analysis, how \textbf{likely} does such a question type occur?
	\item During process analysis, how \textbf{frequently} does such a question type occur?
\end{itemize}
	
% \emph{Usefulness} refers to the result of a query (called the ``answer'' in the interview) using a particular predicate, while \emph{importance} refers to the query itself, both for process analysis purposes.
\emph{Usefulness} and \emph{importance} are two external metrics on data quality \cite{WandWang96}: they focus on the use and effect of an information system (in our case, of a given predicate in the PQL language) addressing the purpose and justification of the system, and its deployment in an organization. While Wand and Wang present a range of external metrics (such as timeliness, flexibility, sufficiency, conciseness), we deemed usefulness and importance to be the most representative ones in our context (assessing the relevance of a given behavioral predicate), in light of the need to keep the interview brief. Internal metrics such as accuracy have been proven formally in this paper. 

We complemented usefulness and importance with \emph{likelihood} and \emph{frequently}, two other data quality metrics which act as proxy of the occurrence of a given predicate during process analysis. More specifically, these latter two metrics measure the \emph{intensity} of using a predicate in an organization, i.e.\ the more likely and frequently a predicate occurs, the more intense is its use \cite{MendlingSR12}. %As such, they complement the other two metrics on data quality by providing insights on the and intensity of use.

In the last part of the questionnaire, we allowed the interviewees to provide any additional comments on these aspects of the PQL language. The complete instrument is provided in Appendix~\ref{app:PQL:interview}. 

% \begin{table}[htbp]
% \footnotesize
%   \centering
% \begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{3cm}|}
% \hline
% How \textbf{useful} would an answer to such a question type be for your process analysis work? & How \textbf{important} is such a question type to your process analysis work? & During process analysis, how \textbf{likely} does such a question type occur? & During process analysis, how \textbf{frequently} does such a question type occur? \\
% \hline
% 1 -- Not at all useful\newline
% 2 -- Slightly useful\newline
% 3 -- Moderately useful\newline
% 4 -- Very useful\newline
% 5 -- Extremely useful
% &
% 1 -- Not at all important\newline
% 2 -- Slightly important\newline
% 3 -- Moderately important\newline
% 4 -- Very important\newline
% 5 -- Extremely important
% &
% 1 -- Extremely unlikely\newline
% 2 -- Unlikely\newline
% 3 -- Neutral\newline
% 4 -- Likely\newline
% 5 -- Extremely likely
% &
% 1 -- Never\newline
% 2 -- Almost never\newline
% 3 -- Occasionally\newline
% 4 -- Almost every time\newline
% 5 -- Always
% \\
% \hline
%     \end{tabular}
%   \label{tab:interview:scale}\caption{Questions used in the empirical assessment of relevance.}\label{tab:questions}
% \end{table}

\subsection{Results}
\label{subsec:empirical:evaluation:results}

We conducted the interviews over a period of three months and obtained a reply from eleven practitioners. One entry was discarded because of inconsistency between the results, leading to a total of ten entries. 

The participants' education is quite varied, ranging from information technology, engineering, accounting and economics, to biology and sociology. Roles include managing director, (senior) manager, business process management (BPM) consultant, BPM/business architect and business analyst. The experience with process model collections varies from 6 months to up to 40 years, with an average of 11 years (stdev = 11.8 years). 

The number of models being managed/analysed in their practice varies from tens to thousands (3,800 models on average, stdev = 10,600). These models belong to different industry verticals: insurance, banking, investments and business recovery, HR, finance and budgeting, procurement, product lifecycle, IT and change management, media and healthcare. The type of models is also quite varied, ranging from simple and structured to large, complex and unstructured models, in the EPCs and BPMN modeling languages. The most recurring problems faced in managing these model collections are related to maintenance and understandability, validation, compliance and standardization.  

\begin{table}[htbp]
\footnotesize
  \centering
\begin{tabular}{r|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-13}
& \rotatebox[origin=l]{90}{\texttt{CanOccur}\;\;} & \rotatebox[origin=l]{90}{\texttt{AlwaysOccurs}\;\;} & \rotatebox[origin=l]{90}{\texttt{Cooccur}\;\;} & \rotatebox[origin=l]{90}{\texttt{Conflict}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistTotalCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalExistCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalCausal}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{ExistTotalConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalExistConcurrent}\;\;} & \rotatebox[origin=l]{90}{\texttt{TotalConcurrent}\;\;} \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Useful} } & 4.0   & 3.6   & 3.7   & 3.7   & 3.3   & 3.4   & 3.6   & 3.9   & 3.0   & 3.2   & 3.6   & 3.9 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Important} } & 3.8   & 3.4   & 3.4   & 3.6   & 3.3   & 3.3   & 3.4   & 3.8   & 3.1   & 3.0   & 3.3   & 3.5 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Likely} } & 4.4   & 3.4   & 3.8   & 3.5   & 2.9   & 3.4   & 3.4   & 3.3   & 3.4   & 3.2   & 3.1   & 3.4 \\
\hline
\multicolumn{1}{ |r|  }{\multirow{1}{*}{Frequent} } & 3.5   & 3.2   & 3.2   & 2.9   & 2.6   & 2.9   & 2.9   & 3.1   & 2.6   & 2.8   & 3.0   & 3.2 \\
\hline
% \hline
% \multicolumn{1}{ |r|  }{\multirow{1}{*}{Sum} }   & \textbf{15.7} & \textbf{13.6} & \textbf{14.1} & \textbf{13.7} & 12.1  & 13.0  & 13.3  & \textbf{14.1} & 12.1  & 12.2  & 13.0    & \textbf{14.0}\\
% \hline
    \end{tabular}
  \label{tab:interview:averages}\caption{Average results of the empirical assessment of the twelve predicates over all participants, per metric.}\label{tab:empirical_results}
\end{table}

Table~\ref{tab:empirical_results} summarizes the results of the predicates assessment along the four metrics chosen (usefulness, importance, likelihood, frequency), averaged over all ten participants (with 1 being very low and 5 being very high, e.g.\ for usefulness 1 = ``Not at all useful'' and 5 = ``Extremely useful'', cf. Appendix~\ref{app:PQL:interview} for full instrument). We  observe that on average all predicates are perceived to be useful, important, likely and frequent, with stronger results for usefulness and importance (average equal or above 3.0). 

%we are 95\% confident that the true value of the parameter is in our confidence interval
%we express that 95% of the hypothetically observed confidence intervals will hold the true value of the parameter

Figure~\ref{fig:confidence} shows the 95\% confidence intervals on the average over the four metrics.\footnote{This chart expresses that 95\% of the hypothetically observed confidence intervals will hold the true value of each predicate.} The results are quite consistent across all predicates, with all intervals and standard deviations being quite low (max 1). The lower bound of all intervals is above 2.5, which is the threshold between a good and a bad predicate assessment. Moreover, the mean is always above 3, signifying a positive perception of the predicate's relevance. In sum, these results confirm the perceived practical relevance of the twelve behavioral predicates for process model querying with our experts group. These results are resonated by the open comments we collected in the last part of the interview, which suggest strong support and encouragement for this line of research on behavioral querying of process model repositories:
    
\begin{quote}
\emph{``[TotalCasual] is actually useful because it links into compliance and governance. So, if you know that within a process for the governance piece to be executed correct, A has to go before B across your models -- such as for validating maybe a person's identification prior to payment -- you'd actually retrieve . For example, you'd have to make sure that the 100 point check is done prior to payment.  So if there's a payment, is there a preceding 100 point check to validate the customer?''.}
\end{quote}
 
%relevance which we define in terms of usefulness, importance, likelihood and frequency of a predicate to be used in practice.

\begin{figure}[t]
\centering
\includegraphics[scale=.6]{confidenceIntervals}
\caption{\label{fig:to:unify}95\% confidence intervals on the weighted average of the assessment of the twelve behavioral predicates over the four metrics of usefulness, importance, likelihood and frequency.}\label{fig:confidence}
\end{figure}

The intention of this experiment was not to claim statistical significance of the results (which is not possible due to the low number of respondents), but to shed light on the relevance of the problem at hand, and to drive the implementation of a selection of these predicates in our language. Accordingly, we selected the six most relevant predicates, namely \emph{CanOccur}, \emph{AlwaysOccurs}, \emph{Cooccur}, \emph{Conflict}, \emph{TotalCausal} and \emph{TotalConcurrent}, on the basis of the results of the 95\% confidence intervals shown in Figure~\ref{fig:confidence}: these six predicates have the highest mean across all twelve predicates (ranging from 3.4 to 3.93), and the highest lower bound of the confidence interval (ranging from 2.93 to 3.38). 

This selection includes the two unary predicates as well as one representative of each of the four categories of behavioral relations (co-occurrence, conflict, causality and concurrency). It is not surprising that the causality and concurrency predicates with the total property were perceived as being more relevant than their existential counterpart (``Exist'', ``ExistTotal'' and ``TotalExist''). The ``total'' version is arguably simpler to understand and to relate to practice (e.g.\ for compliance purposes), since it requires all instances of all process models in a collection to satisfy the behavioral relation captured by the predicate. As an example, the question type we asked for \emph{TotalConcurrent} is ``Find all process models where for \emph{every} instance in which tasks \textbf{A} and \textbf{B} both occur, it holds that \emph{every} occurrence of task \textbf{A} can be executed at the same time with \emph{every} occurrence of task \textbf{B}'', while that for \emph{ExistConcurrent} is ``Find all process models where in \emph{at least one} instance it holds that \emph{some} occurrence of \textbf{A} can be executed at the same time with \emph{some} occurrence of task \textbf{B}'' (cf. Table~\ref{tab:predicates}).









